A Scenario-Oriented Benchmark for Assessing AIOps Algorithms in Microservice Management

AIOps algorithms play a crucial role in the maintenance of microservice systems. Many previous benchmarks' performance leaderboard provides valuable guidance for selecting appropriate algorithms. However, existing AIOps benchmarks mainly utilize offline datasets to evaluate algorithms. They cannot consistently evaluate the performance of algorithms using real-time datasets, and the operation scenarios for evaluation are static, which is insufficient for effective algorithm selection. To address these issues, we propose an evaluation-consistent and scenario-oriented evaluation framework named MicroServo. The core idea is to build a live microservice benchmark to generate real-time datasets and consistently simulate the specific operation scenarios on it. MicroServo supports different leaderboards by selecting specific algorithms and datasets according to the operation scenarios. It also supports the deployment of various types of algorithms, enabling algorithms hot-plugging. At last, we test MicroServo with three typical microservice operation scenarios to demonstrate its efficiency and usability.

==> algorithms/algorithm_py.tex <==
\begin{lstlisting}[caption={Users need to extend an \textit{Algorithm} class in algorithm.py and import their own model methods. We encapsulate AutoMap into the \textit{AutoMap} class, implementing the interfaces for AutoMap training and testing. Therefore, when implementing the \textit{run} method of the \textit{Algorithm} class, we can complete the operation by directly calling \textit{AutoMap.run}, and return the result\_dict from the \textit{run}.},label={lst:algorithm_py}]
from automap.automap import AutoMap
from algorithm_app.public_function import get_config, deal_config
class Algorithm:
    def __init__(self, user):
        config = get_config(config_file)
        config = deal_config(config, user, base_dir)
        self.model = AutoMap(config)
        self.experiment_dir = os.path.join(base_dir, user)
        self.origin_data_dir = os.path.join(base_dir, user, sys_config['origin_data_dir'])

    def run(self):
        try:
            result_dict = self.model.run(self.origin_data_dir)
            print(result_dict)
        except Exception as e:
            print(e)
        finally:
            self.clear()

    def clear(self):
        if os.path.exists(self.experiment_dir):
            shutil.rmtree(self.experiment_dir)
\end{lstlisting}



==> algorithms/config_yaml.tex <==
\begin{lstlisting}[caption={config.yaml of AutoMap},label={lst:config_yaml}]
metric_dir: 'metric'
  
sequence_num: 10

result_path: 'result.json'
\end{lstlisting}

==> sections/benchmark_dataset.tex <==
This section presents an open-source dataset: \datasetname \footnote{Dataset available at: https://github.com/MicroServo/dataset},  a \workname-generated microservice fault dataset that covers all fault types described in Section \ref{sec:fault injection}.
\subsection{Service Topology}
The service topology of \datasetname\ is primarily based on Online Boutique, as Fig \ref{fig:service-topology} shown. An edge directed from Service A to Service B signifies that Service A has sent a request to Service B.

\datasetname\ comprises 11 microservices. The frontend acts as the user-facing front-end of the microservices system that accessible to users,  redis-cart is a Redis database that interacts with the cartservice, and the rest of the services are back-end services. The system uses dynamic deployment. Except for redis-cart, three pods are deployed for each service. These 31 pods are dynamically deployed across 8 virtual machines.

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth, height=0.2\textheight]{figure/topology.pdf}
    \caption{The topology of \datasetname\ microservice system}
    \label{fig:service-topology}
\end{figure}

\subsection{Data Format}

\textbf{Metric}: Same to the types of metrics introduced in Section \ref{sec:data collection}, \datasetname\ includes 17 container-level metrics and 10 service-level metrics, each stored in separate CSV files. The format for these files is as follows: (\textit{timestamp}, \textit{cmdb\_id}, \textit{kpi\_name}, \textit{value}), where each line represents a value sampled from all instances of a service. The sampling frequency is set at 1 second, and users have the flexibility to set the step size of the metrics dataset according to their requirements, with a minimum step size of 1 second.

\textbf{Log}: The logs within \datasetname\ are preserved in a CSV file. Each row in the CSV file corresponds to an individual log entry, representing a singular event or state captured by the microservice's logging system. And the format of the CSV file is composed of the following columns: (\textit{log\_id}, \textit{timestamp}, \textit{date}, \textit{cmdb\_id}, \textit{message}). 
% \textit{cmdb\_id} is the identifier of the microservice instance from which the log was generated. This allows for the tracking of logs on a per-service basis. \textit{message} is the actual message content of the log entry.

\textbf{Trace}: The traces in \datasetname\ is stored in a CSV format, capturing the intricate web of service requests. The CSV file is meticulously structured with columns that consist of: (\textit{timestamp}, \textit{cmdb\_id}, \textit{parent\_span}, \textit{span\_id}, \textit{trace\_id}, \textit{duration}, \textit{type}, \textit{status\_code}, \textit{operation\_name}). 
% \textit{cmdb\_id} refers to the identifier of the specific service instance participating in the trace, crucial for service-level traceability. \textit{parent\_span} denotes the ID of the preceding request in the call hierarchy, linking the trace's continuity. \textit{span\_id} is the unique identifier for the current service invocation within the trace, providing granularity. \textit{trace\_id} is the overarching identifier that aggregates all related spans for a full transaction across the system. \textit{duration} records the execution time for the individual trace, typically in milliseconds, vital for performance analysis. \textit{type} indicates the protocol, such as gRPC or HTTPS, underlining the method of communication. \textit{status\_code} captures the response status for the invocation, shedding light on the outcome. \textit{operation\_name} gives a descriptive label to the operation being performed, essential for identifying the purpose of the trace segment. 
These fields assemble a comprehensive narrative of each trace, invaluable for diagnosing issues, optimizing performance, and understanding the system's behavior under various conditions.

\subsection{Fault Scenarios}
\label{sec:fault scenarios}
\datasetname\ contains seven types of faults, and a wealth of fault scenarios have been designed by varying the duration and intensity of these faults. Table \ref{table:dataset_scenario} lists parts of fault scenarios in \datasetname. 
% Scenario 1, at 2:00, induces a condition where the CPU utilization of paymentservice-1 reaches 100\% for a duration of 15 minutes. Scenario 2, at 4:35, disrupts the connection to the productcatalogservice-2, causing its port 3550 to temporarily cease accepting requests for 13 minutes. In Scenario 3, at 6:23, currencyservice-0 experiences a downtime of 12 minutes. Scenario 4, at 10:20, introduces a unilateral network packet loss of 50\% from recommendationservice-1 to productcatalogservice-1, lasting for 9 minutes. Scenario 5, at 14:50, adds a delay of 3000 milliseconds to requests on port 5050 of checkoutservice-1, persisting for 11 minutes. Scenario 6, at 16:07, fully occupies the memory usage of emailservice-2 for a span of 10 minutes. Finally, Scenario 7, at 20:49, imposes a one\-way network delay of 2000 milliseconds between cartservice-2 and redis-cart-0, lasting for 14 minutes.

\input{tables/dataset_scenario}

==> sections/experiment.tex <==
\subsection{Experiments}
To validate the algorithm hot-plugging functionality of \workname, we deployed AutoMap\cite{automap}, JumpStarter\cite{jumpstarter}, NeuralLog\cite{neurallog}, LogCluster\cite{logcluster}, TraceAnomaly\cite{traceanomaly}, TraceRCA\cite{tracerca}, and DiagFusion\cite{diagfusion} onto \workname. We utilized the datasets generated by \workname\ to run these algorithms and to display their results.

\textit{Experiment setup}. We divided the seven algorithms into two groups. The first group comprised AutoMap, LogCluster, TraceRCA, TraceAnomaly and JumpStarter, which are not split into separate training and testing phases. The second group, including DiagFusion and NeuralLog, are deployed online with the process divided into training and testing phases. Experiments are then conducted for each group.

\textit{Dataset}. Following the fault scenarios described in Section \ref{sec:fault scenarios}, we arrange two days of fault injection. For the first group, the full two-day dataset is used as input. For the second group, we train models using the first day's data as a training set and employ the second day's data for the models to perform detection or diagnosis. The dataset contains 3776976 records in the log and 1278142 records in the trace, with a total of 27 metrics, among which different metrics may have different numbers of records. 

\subsection{Baselines}
\textbf{AutoMap}\cite{automap} is an automated fault diagnosis tool for microservices architectures, using a behavior graph-based method to identify and automatically detect the root causes of faults. 
% This tool combines various performance indicators and advanced model learning techniques to dynamically generate associations between services and automate the diagnostic process. This method enhances the efficiency and accuracy of fault handling, especially suitable for complex microservices environments.

\textbf{JumpStarter}\cite{jumpstarter} uses Compressed Sensing (CS) technology, focusing on anomaly detection in multivariate time series data. 
% This technology allows for signal reconstruction with fewer samples than required by the Nyquist rate, particularly suited for rapid initialization and accurate anomaly detection in online service systems. This method demonstrates efficient performance in real-time system monitoring.

\textbf{LogCluster}\cite{logcluster} focuses on log clustering for problem diagnostics in large online service systems. 
% By clustering log messages, it simplifies the diagnostic process, particularly effective in environments with large and complex data. This method quickly identifies abnormal patterns and potential issues, providing system administrators with a practical tool for monitoring and maintaining system health.

\textbf{NeuralLog}\cite{neurallog} is a deep learning-based log anomaly detection algorithm that uniquely uses raw log messages without relying on traditional log parsing. 
% The algorithm employs the BERT model to semantically encode log data and uses a Transformer-based model to detect anomalies, effectively capturing the contextual information and semantic meanings in the logs, thereby enhancing the accuracy and interpretability of anomaly detection.

\textbf{TraceAnomaly}\cite{traceanomaly} is an unsupervised learning algorithm for microservices call trace anomaly detection. 
% It uses deep Bayesian networks to learn the normal patterns at the service level and automatically identifies deviations within these patterns to detect anomalies. This method combines service call paths and response time patterns, effectively improving the accuracy and explainability of anomaly detection.

\textbf{TraceRCA}\cite{tracerca} is a root cause localization algorithm for microservices systems, identifying the source of issues through the analysis of service call trace data. 
% This algorithm uses trace anomalies to unearth suspicious collections of microservices and ranks these services to accurately locate the root causes of failures, proving to be an effective diagnostic tool, particularly suited for complex microservice environments.

\textbf{DiagFusion}\cite{diagfusion} employs a comprehensive approach, initially extracting events from system traces, logs, and metric data using the fastText algorithm to learn a unified representation of these events. DiagFusion then constructs dependency graphs combining trace and deployment data, utilizing Graph Neural Networks (GNN) to analyze and learn the propagation patterns of system failures.

\subsection{Results}
All baselines' results are shown in Table \ref{table:detection} Table \ref{table:diagnosis}. For algorithms such as AutoMap \cite{automap} and LogCluster \cite{logcluster} that perform poorly, users can continuously modify the algorithm or arrange more complex fault scenarios to fine-tune the model. For algorithms with low training efficiency, such as TraceAnomaly \cite{traceanomaly} and TraceRCA \cite{tracerca}, users can focus on optimizing the training logic of the algorithm and choose datasets from different time periods for an experiment. In summary, MicroServo provides one-stop assistance for evaluating the deployment capabilities of algorithms.

\input{tables/detection}

\input{tables/diagnosis}


==> sections/hot-plugging-2.tex <==
We have contemplated critical questions about how algorithms operate, what their running costs are, and how their effects are demonstrated, which leads to the creation of Algorithm hot-plugging functionality. It is an essential component in the algorithm capability evaluation framework. The choice of the name is self-explanatory: We aim to achieve a platform integration for algorithms as simple as plugging into a socket and just as easily detachable for use anywhere. Below, we present our design philosophy, focusing on providing users a convenient and versatile experience.

\subsection{Implement few Interfaces}
\label{sec:implement-interface}
To facilitate the successful deployment of user-defined algorithms on \workname, we have designed a template known as MicroServo-SDK. Users are required to follow the instructions to enhance the MicroServo-SDK. Its structure is as follows:

\textbf{config.yaml} file is the project's system configuration file, which includes settings such as the paths for original data files. When users write preprocessing code for the original data, they only need to utilize the paths to the raw data files specified in this configuration file.

\textbf{djangoTemplate} is the configuration folder for the project. It contains urls.py, which maps project URLs to view functions, and settings.py, which includes all configurations for the Django project, such as middleware, templates, and static file paths. Users do not need to modify this folder.

\textbf{dockerfile} builds the entire Inputs project into an image. Its base image is python:3.9.

\textbf{docker-compose.yaml} is a configuration file provided for users to test whether their algorithms can run correctly. After completing all the prepare work, executing \textbf{docker compose up} allows the algorithm container to run locally. The functionality of the algorithm can then be verified by sending requests to port 8000 of the container to check if it can train and test properly.

\textbf{requirements.txt} is the dependency file for the project environment. Users need to add their algorithm's requirements.txt into this file.

\textbf{algorithm} folder is used to store the user's own algorithms. 

% \input{algorithms/config_yaml}

\textbf{Algorithm\_app} is a Django application that furnishes interfaces for algorithms. Within it, algorithm.py is dedicated to defining the specific implementation logic of algorithms, while views.py establishes the interfaces awaiting invocation, which are abstracted away from the user's concern. It extends an Algorithm class in algorithm.py. 
% This class encompasses five methods: \textit{\_\_init\_\_}, \textit{train}, \textit{test}, \textit{run}, and \textit{clear}. The \textit{\_\_init\_\_} method is responsible for handling the path information of the algorithm, initializing your model, and providing some variables for the original data and the \textit{clear} method is responsible for cleaning up temporary files after each experiment. The \textit{train} method should include data preprocessing logic, using the preprocessed data to train the model, and saving the model in the experiment path after training is complete. And the \textit{test} method needs to return Json data in a specific format which is explained in Section \ref{sec:evaluation-metric}. \workname\ will store the data in the database and display it on the platform's evaluation data page.

Although the MicroServo-SDK appears complex, users need to perform only two tasks to upload their algorithms to \workname. 

\textbf{Modify code to meet our requirements}. Initially, all file path information must be integrated into a configuration file in the algorithm folder using absolute paths. The naming of keys in the configuration file must also adhere to the following rules: directories end with \_dir and files with \_path. Users must prepare a requirements.txt file detailing all necessary dependencies for the algorithm's execution.

\textbf{Implement the algorithm.py in the algorithm\_app folder}. If users choose to deploy the algorithm online, which means saving the model after the training process, they need to implement the \textit{train} method to train the model and the \textit{test} methods to test it. Alternatively, if they want to observe the effects of the model, they should implement the \textit{run} method, which trains, tests the model, and obtains results in one process.

As for the intricacies of data collection and the storage of experimental results, these details are entirely managed by the system, relieving users of such concerns.

\subsection{One algorithm, One container}
Running two algorithms concurrently within the same environment often leads to issues such as dependency conflicts. To address this problem, we deploy each user-uploaded MicroServo-SDK in separate containers. This approach ensures that each algorithm experiment operates without interfering with others, achieving effective isolation. Furthermore, since algorithms are managed as containers, they can be administered similarly to managing containers. Operations such as adding or deleting an algorithm simply require manipulation of the corresponding container, facilitating these changes efficiently. Additionally, the containers are completely decoupled from the platform, allowing users to upload various algorithms without the hassle of managing them.

\subsection{Online Deployment}
In Section \ref{sec:implement-interface}, the distinction between differentiating training and testing phases and not distinguishing them may indeed need some clarification. Differentiating between training and testing stages is a conventional approach in standard machine learning processes. Specifically, within the \workname\ application scenario, differentiating training from testing implies initially training the model on the platform, then saving the trained model for subsequent testing or practical operations—this is referred to as \textbf{online deployment}.

The advantage of online deployment is that it allows the system to continuously operate the same model, thereby effectively evaluating the model's performance at different times or on different datasets and facilitating iterative updates and refinements. This method not only assesses the training costs of algorithms but also conveniently tests the algorithm's effectiveness across diverse datasets. Additionally, it supports retraining the model to assess long-term maintenance costs or explore its adaptability to new data through incremental learning.

Therefore, the online deployment capability supported by \workname\ significantly enhances the ability to evaluate and apply algorithm performance, especially in complex and dynamically changing practical environments. This feature improves the practicality and flexibility of algorithms and provides researchers and engineers with a powerful tool to optimize and adjust algorithms to meet real-world requirements.

\subsection{Unified Criterion}
\label{sec:evaluation-metric}

We categorize the supported algorithms as AD, RCA, and FC.

\textbf{AD}. Anomaly detection is identifying data points in a dataset or system that are outside the normal range and flagging instances in the data that do not fit a conventional pattern or statistical model.

\textbf{RCA}. Root cause analysis aims to find out the root cause of the failure and locate the entity of the failure, integrate a large amount of data and expertise to improve operations efficiency, and has high research value in the diagnostic microservice architecture

\textbf{FC}. Failure classification is used to classify failures occurring in a system or device. Its goal is to identify and organize failures effectively to better understand the failure mode, quickly locate the problem, and take appropriate measures to solve it.

Additionally, we provide several evaluation metrics for users to choose from to facilitate the comparison of different algorithms' performance.

\textbf{Precision, Recall, and F1-score}. These three metrics are usually used together to assess the performance of classification tasks. 

\textbf{$\text{Accuracy@k}$}. This metric measures whether the correct answer is included in the $top@k$ results predicted by the model. This prediction is considered correct if the correct answer is within the first $k$ answers provided by the model.

\textbf{$\text{Top@k}$}. This metric checks if the target category is included among the $top@k$ predictions of the model. Similar to $Accuracy@k$, it focuses more on whether the model can rank the correct category among the top few in classification tasks.

As visualization of evaluation metrics is necessary, we specify a particular format for each metric. As Listed in Table \ref{tab:evaluation_metrics}, if a user selects the $Top@k$ evaluation metric, they need to organize the experimental results into a JSON format with keys $top@k$ and $epoch$, where $i$ indicates the result of the $i$-th epoch.

\input{tables/evaluation_metric}

==> sections/hot_plugging.tex <==
Algorithm hot-plugging is the highlight of \workname. It deploys each algorithm in a distinct Docker container\footnote{https://www.docker.com/resources/what-container/} to execute experiments, with the outcomes stored in a database. This method benefits from the isolation of running environments for each algorithm, avoiding dependency conflicts. Moreover, by decoupling the algorithms from the \workname, it facilitates the convenient operation and comparison of varying algorithms and their respective results.

The architecture and the communication pathways among components in two common use-cases are depicted in Fig.~\ref{fig:hot-plugging} as presented in \workname.

When user uploads MicroServo-SDK through the API interface, Docker container controller initiates the creation of a new container. Within this container, a Django\footnote{https://www.djangoproject.com/} server is started, exposing interfaces for the training and testing of the algorithm, while continuously listening on port 8000. If user invokes the API for running expriment, Docker container controller first collects data from Elasticsearch. Once data collection is complete, the controller invokes the interface of the specified algorithm container, mounting data within the container, thus officially commencing the algorithm experiment. Upon completion of the experiment, the results are stored in the MySQL\footnote{https://www.mysql.com/} database in JSON format.


\subsection{MicroServo-SDK}
\label{sec:algorithm-inputs}
To facilitate the successful deployment of user-defined algorithms on \workname, we have designed a template known as MicroServo-SDK. Users are required to follow the instructions to enhance the MicroServo-SDK. Its structure is as follows:

\textbf{config.yaml} file is the project's system configuration file, which includes settings such as the paths for original data files. When users write preprocessing code for the original data, they only need to utilize the paths to the raw data files specified in this configuration file.

\textbf{algorithm} folder is used to store the user's own algorithms. Before starting implementing the training and testing methods for the algorithm, user needs to make some modifications to the code to meet our requirements. Initially, all file path information must be integrated into a configuration file at the algorithm folder, using absolute paths. Additionally, the naming of keys in the configuration file must adhere to the following rules: directories end with \_dir and files with \_path. As depicted in Listing \ref{lst:config_yaml}, result\_path is the path to the result file, hence the \_path suffix; metric\_dir indicates a directory of metric files, ending with \_dir; while sequence\_num is the parameter thus no suffix added. Subsequently, users must prepare a requirements.txt file detailing all necessary dependencies for the algorithm's execution. Lastly, an optional but recommended step: optimizing the algorithm code by encapsulating the logic within train and test methods, which facilitates the creation of interfaces later on.

\input{algorithms/config_yaml}

\textbf{algorithm\_app} is a django application that provides interfaces for algorithms. A crucial file that users need to implement is algorithm.py. As exemplified in Listing \ref{lst:algorithm_py}, it imports the AutoMap\cite{automap} class defined within the algorithm module and further extends an Algorithm class. This class encompasses five methods: \textit{\_\_init\_\_}, \textit{train}, \textit{test}, \textit{run}, and \textit{clear}.

The \textit{\_\_init\_\_} method is responsible for handling the path information of the algorithm, initializing your model, and providing some variables for the original data. If users choose to deploy the algorithm online, they need to implement the \textit{train} method to train the model and the \textit{test} methods to test it. The \textit{train} method should include data preprocessing logic, using the preprocessed data to train the model, and saving the model in the experiment path after training is complete. And the \textit{test} method needs to return Json data in a specific format which is explained in Section \ref{sec:evaluation-metric}. \workname\ will store the data in the database and display it on the platform's evaluation data page. Alternatively, if users just want to observe the effects of the model, they should implement the \textit{run} method, which train, test the model, and obtain results in one process. Lastly, the \textit{clear} method is responsible for cleaning up temporary files after each experiment.

\textbf{djangoTemplate} is the configuration folder for the project. It contains urls.py, which maps project URLs to view functions, and settings.py, which includes all configurations for the Django project, such as middleware, templates, and static file paths. Users do not need to modify this folder.

\textbf{dockerfile} builds the entire Inputs project into an image. Its base image is python:3.9.

\textbf{docker-compose.yaml} is a configuration file provided for users to test whether their algorithms can run correctly. After completing all the prepare work, executing \textbf{docker compose up} allows the algorithm container to run locally. The functionality of the algorithm can then be verified by sending requests to port 8000 of the container to check if it can train and test properly.

\textbf{requirements.txt} is the dependency file for the project environment. Users need to add their algorithm's requirements.txt into this file.

\subsection{Docker container controller}
Docker container controller is responsible for the deployment, start-up, and management of containers. Depending on the function, it accepts two types of inputs. For deploying a container, it takes the MicroServo-SDK introduced in Section \ref{sec:algorithm-inputs} as input. After storing the input, it uses the Python Docker library to build an image and run the container, finally registering it at the controller. For managing containers, it accepts the container ID as input, locates the specific container, and executes a series of commands such as restart and delete. Information related to the containers is stored in the MySQL database.

Regarding each specific container, they all run a simple Django backend inside, listening on port 8000, awaiting invocation. When the controller receives a request of running experiment, such as using one algorithm to detect a period of data, the controller sends request to specific container, and the backend inside the container executes the detecting method. Once the detection is complete, the results are stored in the MySQL database.

\subsection{Outputs and Evaluation Metrics}
\label{sec:evaluation-metric}
\workname\ categorizes the supported algorithms as: AD, RCA, and FC.

\textbf{AD}. Anomaly detection is the process of identifying data points in a dataset or system that are outside the normal range, and flagging instances in the data that do not fit a conventional pattern or statistical model.

\textbf{RCA}. Root cause analysis aims to find out the root cause of the failure and locate the entity of the failure, integrate a large amount of data and expertise to improve operations efficiency, and has high research value in the diagnostic microservice architecture

\textbf{FC}. Failure classification is used to classify failures occurring in a system or device. Its goal is to identify and organize failures effectively, so as to better understand the failure mode, quickly locate the problem, and take appropriate measures to solve the problem.

Additionally, to facilitate the comparison of different algorithms' performance, \workname\ also provides several evaluation metrics for users to choose from.

\textbf{Precision, Recall, and F1-score}. These three metrics are usually used together to assess the performance of classification tasks. 

\textbf{$\text{Accuracy@k}$}. This metric measures whether the correct answer is included in the $top@k$ results predicted by the model. If the correct answer is within the first $k$ answers provided by the model, this prediction is considered correct.

\textbf{$\text{Top@k}$}. This metric checks if the target category is included among the $top@k$ predictions of the model. Similar to $Accuracy@k$, but it focuses more on whether the model can rank the correct category among the top few in classification tasks.

As visualization of evaluation metrics is necessary, \workname\ specifies a particular format for each metric. As Listed in Table \ref{tab:evaluation_metrics}, if a user selects the $Top@k$ evaluation metric, they need to organize the experimental results into a JSON format with keys $top@k$ and $epoch$, where $i$ indicates the result of the $i$-th epoch.

\input{tables/evaluation_metric}

==> sections/introduction_2.tex <==
Microservice architecture, which utilizes loosely coupled and independently scalable services, has revolutionized the development and deployment of web applications\cite{microservice-architecture}. This architectural model is widely adopted due to its ability to enhance agility, improve scalability, and facilitate continuous deployment, making it ideal for businesses that need to update and scale components frequently. Nowadays, more and more companies migrate to microservice architecture; for example, Netflix's online service system \cite{netflix2018} uses about 500+ microservices, and Tencent's WeChat system \cite{wechat2018} accommodates more than 3,000 services running on over 20,000 machines \cite{trainticket}.

When a system encounters a failure, to avoid excessive losses, enterprises need the ability to quickly detect anomalies (Anomaly Detection, AD), classify the failure (Failure Classification, FC), and locate the root cause (Root Cause Analysis, RCA). However, due to the complex structure of microservice systems, relying solely on manual efforts is insufficient.
 Therefore, researchers have utilized three types of data that reflect system states: application logs\cite{log}, performance metrics\cite{metrics}, and decentralized traces\cite{traces}, to develop many algorithms such as \cite{automap,diagfusion,jumpstarter,logcluster,tracerca,traceanomaly,neurallog}. This paper collectively refers to these algorithms as \textbf{AIOps algorithms}. Given the good performance of these AIOps algorithms, enterprises are increasingly willing to apply them to actual production environments.

 To facilitate the deployment of AIOps algorithms into production environments, a comprehensive lifecycle capability evaluation framework is urgently needed. The framework focuses on four key issues:

\textbf{Collection of Failure Cases}: For enterprises that have not established mature system monitoring, collecting real failure data is very challenging. We need to reproduce key failure scenarios in a livebenchmark environment to accurately assess the performance of the algorithm, while providing large and diverse datasets, including application logs, performance metrics, and decentralized traces.

\textbf{Algorithm Training}: At this stage, we focus on the time cost associated with data collection and offline training, as well as the efficiency of algorithm training.

\textbf{Effectiveness of Online Deployment}: After deployment, the model needs to be evaluated for its actual performance to ensure it can operate effectively in a real environment and deliver the expected business value. This stage requires attention to the model's prediction accuracy, response time, and consumption of system resources.

\textbf{Cost of Long-term Maintenance}: Long-term maintenance of the model includes degradation assessment and update evaluation, such as changes in model effectiveness and the cost of retraining data.


In the field of AIOps, there are some commonly used benchmarks available for evaluating microservice systems:

\begin{enumerate}
    \item VECROsim\cite{vecrosim}, which simulates faults in microservices and collects performance metrics on system behavior, mainly focuses on collecting performance metric data, with limited types of fault injection, primarily handling simple fault scenarios such as CPU overload or memory leaks, which cannot adequately represent the complex fault conditions found in production environments.
    \item TrainTicket\cite{trainticket}, a benchmark that includes a variety of microservices for a train ticket booking system, provides real-world scenarios for fault diagnosis studies includes rich data types (such as logs, performance metrics, and trace data), but its fault types are predefined and cannot be customized, limiting its practicality in specific experiments.
    \item µBench\cite{mubench}, an open-source benchmarking tool designed to create and run highly customizable microservice applications for performance evaluation of cloud and edge computing platforms, performs well in customizing microservice applications and fault injection, but like the benchmarks above, it falls short in the aspect of real-time AIOps algorithm deployment.
\end{enumerate}

Although these tools each have strengths, they are generally insufficient to meet the needs of a comprehensive lifecycle capability evaluation for enterprise operations.

To address the above needs, we develop \workname\footnote{We have open-sourced the \workname\ code, which is available at https://github.com/MicroServo/microservo. Additionally, we provide a demo at microervo.aiops.cn for users to try out.}. The term \textit{MicroServo} combines \textit{micro} from microservices and \textit{servo} from servo systems, which implies that the system is designed to provide accurate and detailed evaluations, much like a servo system provides precise control in engineering applications. \workname\ provides a comprehensive evaluation framework for enterprises by integrating multiple data collection, fault injection, and online AIOps algorithm deployment. Specifically, \workname\ has the following core functionalities:

\begin{enumerate}
    \item Multimodal Data Collection: \workname\ can simultaneously collect logs, traces, and performance metrics, providing a comprehensive data view.
    \item Custom Fault Injection: It supports various types of fault injection and is capable of reproducing a wide range of fault scenarios in real environments.
    \item Algorithm hot-plugging: \workname\ supports executing algorithms of types AD, FC, and RCA. Upon uploading an algorithm to the platform, users can select a dataset to train their models. They also have the option to use real-time data to assess the effectiveness of the models. Additionally, users can alter the severity of faults to test the sensitivity of the algorithms to different degrees of failure. This functionality enhances the platform's utility by enabling a comprehensive algorithm performance evaluation under varied conditions.
\end{enumerate}

Our main contributions are as follows:

\begin{enumerate}
    \item We develop \workname,  which establishes a comprehensive lifecycle evaluation framework that spans from data preparation and model training to model testing and online deployment. This framework serves as an instrumental tool to facilitate the implementation of algorithms in the industry.

    \item we design rich fault scenarios in \workname\ to generate and release a collection of multimodal datasets.
\end{enumerate}

==> sections/new_introduction.tex <==
 Microservice architecture, which utilizes loosely coupled and independently scalable services, has revolutionized the development and deployment of web applications\cite{microservice-architecture}. This architectural model is widely adopted due to its ability to enhance agility, improve scalability, and facilitate continuous deployment, making it ideal for businesses that need to innovate quickly. For example, Netflix's online service system \cite{netflix2018}  use about 500+ microservices and handles about two billion API requests every day. And Tencent's WeChat system \cite{wechat2018} accommodates more than 3,000 services running on over 20,000 machines \cite{trainticket}. However, the decentralized nature of microservices introduces complexities in monitoring and maintaining service consistency across distributed systems\cite{microservice-challenge}. These challenges necessitate more sophisticated strategies to manage the intricate interactions and dependencies effectively.

 To tackle the operational challenges introduced by microservice architectures, researchers utilize application logs\cite{log}, performance metrics\cite{metrics}, and distributed traces \cite{traces} collected from microservice systems to perform anomaly detection, fault detection, and fault diagnosis. To date, recognizing the limitations of unimodal approaches, researchers have proposed some multimodal algorithms to enhance fault detection and diagnosis capabilities by leveraging diverse data types, such as Diagfusion\cite{diagfusion}, Eadro\cite{eadro}. In parallel, the community has also developed and released several multimodal datasets like TrainTicket dataset\footnote{https://zenodo.org/records/7615394}, GAIA\footnote{https://github.com/CloudWise-OpenSource/GAIA-DataSet}, AIOps Challenge 21, AIOps Challenge 22, to facilitate research in this area. Through our analysis, we have identified certain limitations in widely-used datasets. The GAIA dataset, although large in volume, suffers from imbalanced fault injection and a limited variety of faults. The TrainTicket dataset, on the other hand, has been found to contain issues with timezone inconsistencies. As a result, the availability of high-quality open-source datasets for researchers remains limited.

 To further customize and generate diverse multimodal datasets, benchmarks specifically designed for microservice architectures have been developed. Notable among these are VECROsim\cite{vecrosim}, which simulates faults in microservices and collects performance metric on system behavior, TrainTicket\cite{trainticket}, a benchmark that includes a variety of microservices for a train ticket booking system, providing real-world scenarios for fault diagnosis studies, and µbench\cite{mubench}, an open-source benchmarking tool designed to create and run highly customizable microservice applications for performance evaluation of cloud and edge computing platforms. These benchmarks are crucial for advancing research in operational management and diagnostics in complex microservice environments. However, they still have limitations. For instance, VECROsim focuses primarily on collecting performance metric data and the types of faults that can be injected are quite limited. For example, VECROsim predominantly handles simple fault scenarios like CPU overload or memory leaks, which may not fully represent the complex fault conditions found in production environments. On the other hand, TrainTicket collects a broader range of data types including logs, performance metrics, and traces, which enriches the dataset for fault diagnosis, however, the types of faults in TrainTicket are predefined and cannot be customized, limiting its utility for experiments that require specific fault scenarios. Although µBench performs well in customizing microservice applications and fault injection, we aim to achieve more.

We aim to develop a comprehensive framework for evaluating capabilities throughout the entire lifecycle of applications based on real enterprise cases—from model (algorithm) training and deployment to long-term maintenance. This framework will provide benchmarks for implementing models in scenarios that closely mirror real-world conditions. It includes functionalities tailored to the key issues enterprises face at various stages of using AIOPS tools, such as initial data requirements, ease of model training and tuning, effectiveness after deployment, and the ongoing costs of long-term maintenance.

 Therefore, we developed \workname\footnote{https://github.com/MicroServo/microservo}, a benchmark based on microservice systems that can collect tri-modal data, custom inject various types of faults, and supports online deployment of algorithms. The term \textit{MicroServo} combines \textit{micro} from microservices and \textit{servo} from servo systems, which implies that the system is designed to provide accurate and detailed evaluations, much like a servo system provides precise control in engineering applications. Additionally, we have released a collection of dataset, which replicates enterprise pain point cases in the LiveBenchmark environment. The fault scenarios cover multiple layers of the system, including network, configuration, and infrastructure. 

 As previously mentioned regarding the key challenges faced by enterprises, the initial data preparation is the first critical issue. \textit{MicroServo} provides functionalities such as custom fault injection and data export capabilities. Secondly, for model training, \textit{MicroServo} allows users to upload their algorithmic models and train them using data from \textit{MicroServo}, providing a series of basic metrics to demonstrate the effectiveness of the models. Lastly, for long-term maintenance, \textit{MicroServo} also supports the online deployment of models, enabling researchers to conduct evaluations of model degradation and updates.
 
 Specifically, our contributions are as follows:

\begin{enumerate}
    \item We develop \workname\ focused on providing datasets with three modalities (logs, traces, and performance metrics) under custom fault scenarios, alongside facilities for online deployment of algorithms.

    \item we design rich fault scenarios in \workname\ to generate and release a collection of multimodal datasets.
\end{enumerate}



==> sections/related_work.tex <==
\subsection{Benchmark Microservice Systems}
\input{tables/benchmark_system}
\input{tables/baseline}
We review some open-source benchmark microservice systems that target different research purposes. µBench\cite{mubench}, is tailored for creating dummy microservice applications on Kubernetes clusters. It allows customizable simulations to assess cloud/edge computing platforms, offering the ability to test various service mesh topologies and microservice behaviors. VECROsim\cite{vecrosim} stands as a multi-dimensional, metric-oriented microservice fault simulation system. It enables crafting on-demand fault scenarios within customizable service topologies and the automated gathering of intricate performance metrics. The comprehensive suite known as DeathStarBench\cite{deathstar} encapsulates an array of services from social networking to banking, embodied within microservices developed across various languages. It intends to dissect the impact of microservices through the layers of cloud and edge systems, utilizing both RPC and RESTful APIs for diverse application behaviors and workloads. TrainTicket\cite{trainticket}, a medium-sized benchmark system, specializes in train ticket booking. It employs Java and JavaScript across its 41 microservices to replicate authentic software engineer-reported incidents through hard-coded faults, thus aiding in system debugging and analysis. As a scalability benchmarking tool, Theodolite\cite{theodolite} evaluates stream processing engines within microservice architectures. It orchestrates experiments to deduce the scalability of systems under varied workloads, addressing the requirements of distributed stream processing engines with substantial efficiency.

Table \ref{table:benchmark_system} compares \workname\ with these mentioned microservice benchmark systems. Among them, µBench and \workname\ stand out for their comprehensive fault injection and data collection capabilities across multiple modalities. Moreover, \workname\ differentiates itself by emphasizing algorithm hot-plugging, allowing for real-time dynamic adaptations, which is critical for environments that require rapid response to changing conditions and fault scenarios.

\subsection{Online Deployment}
Table \ref{table:baseline} discusses various methodologies and compares their ability to be deployed online. DiagFusion\cite{diagfusion} combines RCA and FC, focusing on microservices systems. It leverages data from logs, traces, and metrics to diagnose issues and is capable of realtime diagnosis, making it effective for online deployment in dynamic environments. Eadro\cite{eadro} integrates AD and RCA, utilizing logs, traces, and metrics to tackle faults in microservices. Unlike DiagFusion, it does not mention online deployment capabilities, which may limit its immediate applicability in live system monitoring. AutoMap\cite{automap} applies RCA techniques to metric data to automate the diagnosis of web applications. However, there is no mention of its ability to be deployed online. JumpStarter\cite{jumpstarter} specializes in metric data and is noted for its realtime detection capability, making it well-suited for online deployment in environments requiring immediate feedback. NeuralLog\cite{neurallog} focuses on log data for anomaly detection and does not explicitly support online deployment. LogCluster\cite{logcluster} processes log data and is capable of realtime diagnosis. TraceAnomaly\cite{traceanomaly} uses trace data to detect anomalies and supports realtime detection. TraceRCA\cite{tracerca} detects anomalies in realtime and diagnoses them online.

Online deployment enables these algorithms to test their performance in real-world operational settings, ensuring they can effectively manage and mitigate realtime issues. Therefore, these algorithms must undergo rigorous online deployment testing before full-scale implementation. This step verifies their functional capabilities and ensures that they can operate seamlessly within the dynamic environments for which they are designed, thereby reducing downtime and enhancing system reliability and user satisfaction. Such preparatory measures are essential for leveraging the full potential of advanced monitoring and diagnostic tools in live production environments.


==> sections/system_design.tex <==
\subsection{Architecture}
\label{sec:architecture}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.9\linewidth, height=0.4\textheight]{figure/framework.pdf}
    \caption{Architecture of \workname. \workname\ consists of four modules: a) Microservice System Deployment, b) Data Collection, c) Fault Injection, and d) User Interface and API. Module a) includes clusters, microservice systems, and traffic generation. Module b) comprises observational data collection tools, with data sourced from the microservice systems deployed in module a). Module c) is a fault injection tool targeting various components of the microservice system. Module d) features our designed API interface, offering users comprehensive functionalities such as data monitoring, fault injection, and AIOps algorithm deployment.}
    \label{fig:platform-framework}
\end{figure*}

\workname, which is grounded in microservice systems and associated observation tools, provides practical features such as data monitoring, fault injection, and AIOps algorithms hot-plugging. Fig.~\ref{fig:platform-framework} outlines the architecture of \workname, consisting of four modules:

\begin{enumerate}
    \item Microservice System Deployment: The microservice system is deployed on Kubernetes\footnote{https://kubernetes.io/}. We use a load generator to generate continuous user requests to the frontend of the microservice system, simulating a production environment.

    \item Data Collection: A suite of collection tools is employed to gather three types of data from the microservice system: performance metrics, logs, and traces. This data is automatically processed into a labeled dataset for analysis and modeling.

    \item Fault Injection: Leveraging Chaosmesh\footnote{https://chaos-mesh.org}, fault injection is implemented at both the service and pod levels within the microservice system, enabling thorough testing and resilience assessment.

    \item User Interface (UI) and API: Centering on the execution of AIOps algorithms, we designed a series of convenient interfaces for data monitoring, fault injection, uploading AIOps algorithms, and running experiments.
\end{enumerate}

\subsection{Microservice System Deployment}
\label{sec:microservice deploy}

\textbf{Kubernetes} is a well-known production-grade container scheduling and management system to run containered applications\cite{vecrosim}. \workname\ uses Kubernetes Pods\footnote{https://kubernetes.io/docs/concepts/workloads/pods/} as its basic microservice deployable unit. For the deployment of various components within \workname, we utilize Kubectl\footnote{https://kubernetes.io/docs/reference/kubectl/}, which is a command-line tool for controlling Kubernetes clusters, and Helm\footnote{https://github.com/helm/helm}, a package manager that simplifies the deployment of applications on Kubernetes. 
% To organize and isolate resources, we adopt the concept of namespaces within Kubernetes. This allows for a segregated environment where resources and network policies can operate without interference from other namespaces.In \workname, microservices, observation tools, and fault injection tools are all installed within their respective namespaces. Minikube is chosen for its simplicity and lightweight footprint, offering researchers an easy and cost-effective way to deploy Kubernetes locally for development and testing purposes.

\textbf{Online Boutique}\footnote{https://github.com/GoogleCloudPlatform/microservices-demo} is a demo microservices provided by GoogleCloudPlatform where users can browse items, add them to the cart, and purchase them. It has twelve components. Among these components are ten stateless microservices, one load generator microservice, and one storage service. Online Boutique is an exemplary platform for developers to master contemporary cloud-native deployment techniques within a true-to-life application setting. It has also been used as a microservice benchmark for experiments in \cite{onlineboutique}. In \workname, we set up three instances for each of the ten stateless components, randomly deployed across eight servers.

However, a notable limitation in the Online Boutique's architecture is the frontend service, which is constructed using Go to build the web interface and operates on an HTTP server, while the system's other components are gRPC servers. This difference in protocols creates a challenge for Elastic APM\footnote{https://github.com/elastic/apm-server}, which fails to trace requests within the frontend service, resulting in incomplete call chains. To address this issue, we introduce an additional gRPC server within the frontend service, acting as an intermediary between the HTTP server and the other microservices' gRPC servers. The requests that were initially dispatched directly from the frontend's HTTP server to the other gRPC servers are now routed through the frontend's new gRPC server. This modification allows Elastic APM to successfully trace the requests within the frontend service, thereby enabling the collection of complete call chain data. This strategic enhancement not only rectifies the tracing discrepancies but also improves the overall observability within the system.

\textbf{Locust}\footnote{https://locust.io} is an open-source load testing tool that simulates user behavior to test the performance of web applications. Written in Python, it allows developers to write test scenarios using straightforward Python code. 
% In our case, we utilize Locust to simulate six different types of user requests to assess the performance of our system under load. We configure Locust to spawn 20 concurrent 'users' that interact with the system, each performing a predefined set of actions that a typical user might take. By leveraging Locust, we can emulate a realistic load on our system, which is crucial for data collecting.



\subsection{Data Collection}
\label{sec:data collection}

\textbf{Metric}: We harness Istio\footnote{https://istio.io} and Prometheus\footnote{https://prometheus.io} to gather metrics from the microservice system. Prometheus's powerful querying language and time-series database make it particularly well-suited for storing, querying, and alerting on time-series metrics. The metrics are categorized into two types: \textit{service-level} and \textit{container-level}.

\textit{Service-level metrics}. Istio collects service-level metrics by using its sidecar proxies, which are based on Envoy. When Istio is integrated into a Kubernetes cluster, it automatically injects an Envoy proxy as a sidecar container in the pod of each deployed microservice. These sidecar proxies intercept and control all network communication between microservices. Table \ref{table:service_metrics} lists the supported service-level metrics of \workname.

\input{tables/service_level_metric}

\textit{Container-level metrics}. Table \ref{table:container_metrics} lists the \workname-supported container-level metrics. In \workname, we leverage the cAdvisor tool embedded in the kubelet of Kuberneters to collect container-level metrics. This cAdvisor\footnote{https://github.com/google/cadvisor} instance runs as a daemon, continuously gathering and reporting detailed information on the operational status of containers. The service exposes a metrics endpoint from which Prometheus scrapes data, ensuring a consistent flow of monitoring information. Subsequently, Prometheus is responsible for the aggregation and storage of these metrics. Then we execute Prometheus queries and save them as CSV (comma-separated values) files.

\input{tables/container_level_metric}

\textbf{Log}: We deploy Filebeat\footnote{https://github.com/elastic/beats} for log collection in our microservice environment. Filebeat is configured to capture logs from each pod, efficiently forwarding them to Logstash\footnote{https://github.com/elastic/logstash}. Logstash acts as a centralized log processing pipeline that further refines and aggregates the logs. The processed logs are then directed to Elasticsearch\footnote{https://github.com/elastic/elasticsearch} , a scalable search engine, where they are stored and indexed, making the data readily searchable and analyzable for various operational insights.

\textbf{Trace}: For collecting trace data across our microservices, we use Elastic APM's agents. Given that our microservice architecture is built using multiple programming languages such as Java, Go, C\#, Python, and Node.js, we deploy the respective agents for each technology stack. 
% Python, Node.js and Go agents are intrusive, meaning they may require modifications to the service code or deployment configuration to actively capture the trace data. The others are non-intrusive and can collect data without any code changes, simply by monitoring communication between services. Once deployed, these agents capture detailed request traces  and send them to Elasticsearch. 
To enhance our ability to diagnose and troubleshoot issues, our trace collection focuses on gathering data with method-level granularity. This method-level trace data is valuable for deep performance analysis and understanding the intricate behaviors of complex distributed systems.


\textbf{Elasticsearch and Kibana}: We use Elasticsearch to store both log and trace data, capitalizing on its powerful indexing and search capabilities\cite{elasticsearch}. To facilitate interaction with Elasticsearch, we employ the Elasticsearch library for Python, enabling our developers to programmatically query and manipulate the data according to the needs of our applications and analysis. Additionally, we use Kibana\footnote{https://github.com/elastic/kibana} to manage and interact with Elasticsearch. Kibana provides a user-friendly web interface that makes it easier to visualize, manage, and analyze data stored in Elasticsearch.


\subsection{Fault Injection}
\label{sec:fault injection}
\textbf{Chaos Mesh}: For fault injection, we utilize Chaos Mesh, a powerful cloud-native chaos engineering platform that helps simulate various types of faults and experiments to test the resilience of systems in production-like environments. This tool is particularly useful for verifying system stability under adverse conditions. However, despite its robust capabilities, we identified areas for user interface improvement in Chaos Mesh. Chaos Mesh's default interface uses a list format, making it challenging to observe and manage existing fault orchestrations. The operation can also be quite cumbersome. To address these issues, we redesigned the interface in \workname. Our new design selects a calendar format to provide an intuitive view of fault orchestrations, detailing when and where each fault will occur. We also streamlined the fault injection process to simplify user interactions, making planning and executing chaos experiments more straightforward and less time-consuming. This enhancement significantly improves the tool's usability, facilitating more efficient and effective chaos engineering practices. 

Table \ref{table:fault_injection} summarizes the faults supported by \workname. \workname\ supports injecting five types of faults: CPU, memory, HTTP, pod, and network. Additionally, we offer two modes of fault injection: real-time and scheduled. Users simply need to select the type of fault, the parameters that define the fault's severity, and the target for fault injection. \workname\ will then generate the corresponding YAML file. Upon sending this YAML file to the Chaos Mesh controller, the specified fault is injected as per user requirements. We have also conducted analyses and validations for each type of fault, summarizing how they manifest across three categories of data, as detailed in Table \ref{table:fault_affection}.

\input{tables/chaos_mesh}

\input{tables/fault_affection}


\subsection{UI and API}
\label{sec:user interface}

UI and API components of \workname are meticulously designed around three core functionalities: data monitoring, fault injection, and AIOps algorithm shot-plugging. This design is aimed at providing a user-friendly and convenient operational experience. The front end of \workname\ is built using the Vue 2 framework, incorporating the Element UI component library. On the backend, we have opted for the Django framework, offering RESTful API interfaces that enable efficient communication between the front end and the server. Due to space limitations, we are not displaying the \workname\ page here. You are welcome to visit the \workname\ demo for an experience.


\subsubsection{Inject fault}
In the fault injection page, we use a calendar map format to visually display the historical fault records and the arranged fault scenarios. We currently support various fault types, including network-related, HTTP-related, pod-related, memory load, and CPU load. Users can complete a fault injection operation by clicking on a fault type, selecting the target, adjusting the severity of the fault (such as delay and rate), and setting the execution mode (once or cyclic) and timing. In the calendar map, different colors correspond to different types of faults, and the height of a card represents the duration of the fault. Detailed fault information can be viewed by hovering the mouse over the mini-card. By clicking on a future arranged fault card, you can also choose whether to delete it. In future work, we will integrate more types of faults to help you better arrange more realistic fault scenarios.

\subsubsection{Monitor data}
The data monitoring page provides a way for users to verify the faults they inject by displaying historical fault records, logs, traces, and metrics. We can filter log entries by pod name or message or view the specific fields of each entry. In the metric module, we can select the metrics we want to display. In terms of format, we have adopted the Prometheus style, in which each metric appears in a separate window and the time range can be adjusted independently. Regarding the traces, similar to SkyWalking\footnote{https://github.com/apache/skywalking}, the left side displays the traces while the right side shows specific span information of the trace. This setup allows for a clear visualization of call latency. In addition, we also display the topology information of the microservice system. After verification, the user can click the export button on each module to download the dataset.

\subsubsection{Upload algorithm \& Run experiment}
The two crucial functionalities are depicted in Fig.~\ref{fig:hot-plugging} as presented in \workname.

When a user uploads MicroServo-SDK\footnote{We design a template called MicroServo-SDK for algorithm hot-plugging, available at https://github.com/MicroServo/hot-plugging} through the API interface, the Docker container controller initiates the creation of a new container. Within this container, a Django\footnote{https://www.djangoproject.com/} server is started, exposing interfaces for the training and testing of the algorithm, while continuously listening on port 8000. If the user invokes the API to run an experiment, the Docker container controller first collects data from Elasticsearch. Once data collection is complete, the controller invokes the interface of the specified algorithm container, mounting data within the container, thus officially commencing the algorithm experiment. Upon completion of the experiment, the results are stored in the MySQL\footnote{https://www.mysql.com/} database in JSON format.

\begin{figure*}
    \centering
    \includegraphics[width=1.0\linewidth, height=0.4\textheight]{figure/hot-plugging.pdf}
    \caption{Architecture of Hot-plugging. The algorithm hot-plugging provides users with two functionalities: algorithm upload and experimental execution. The solid arrow represents the process of algorithm upload, where the user completes the Microservo-SDK and then uploads it as input to the platform. Subsequently, the platform deploys it as a Docker container on the server. The dashed arrow represents the process of running experiments; users select an algorithm and dataset and set the execution time. After the platform collects the data, it sends it to the designated algorithm container and then sends a request to run the experiment. Upon receiving the request, the container starts the detection using the model, and after the detection is complete, it stores the results in the database.}
    \label{fig:hot-plugging}
\end{figure*}

==> tables/baseline.tex <==
\begin{table}[h]
    \centering
    \caption{Comparison of Different Baselines}
    \resizebox{\linewidth}{!}{
        \begin{threeparttable}
        \begin{tabular}{llll}
        \toprule
        \textbf{Name} & \textbf{Algorithm Type} & \textbf{Data Modality} & \textbf{Online Deployed} \\
        \midrule
        DiagFusion\cite{diagfusion} & RCA\tnote{1}, FC\tnote{2} & Log, trace, metric & capable of realtime diagnosis \\
        Eadro\cite{eadro} & AD\tnote{3}, RCA & Log, trace, metric & - \\
        AutoMap\cite{automap} & RCA & Metric & - \\
        JumpStarter\cite{jumpstarter} & AD & Metric & capable of realtime detection \\
        NeuralLog\cite{neurallog} & AD & Log & - \\
        LogCluster\cite{logcluster} & Log Cluster & Log & capable of realtime diagnosis \\
        TraceAnomaly\cite{traceanomaly} & AD & Trace & capable of realtime detection \\
        TraceRCA\cite{tracerca} & RCA & Trace & capable of online diagnosis \\
        \bottomrule
        \end{tabular}
        \begin{tablenotes}[para]
            \item[1] Root Cause Analysis (RCA)
            \item[2] Failure Classification (FC)
            \item[3] Anomaly Detection (AD)
        \end{tablenotes}
        \end{threeparttable}
    }
    \label{table:baseline}
\end{table}

==> tables/benchmark_system.tex <==
\begin{table*}[h]
    \centering
    \caption{Comparison of \workname\ with Previous Microservice Benchmarking Systems}
    \resizebox{\linewidth}{!}{
        \begin{threeparttable}
        \begin{tabular}{cccccccccc}
        \toprule
        \multirow{2}[0]{*}{Name}
        & \multicolumn{3}{c}{Microservice System}
        & \multicolumn{3}{c}{Fault Simulation\tnote{1}}
        & \multicolumn{3}{c}{Data Collection\tnote{3}}\\
        \cmidrule(lr){2-4}
        \cmidrule(lr){5-7}
        \cmidrule(lr){8-10}

        & Topology\tnote{2} & Service Type & Language & Injection & Duration & Fault Type & Metric & Log & Trace\\
        \midrule
        \workname\ & M(11) & Online Shopping & Go, Python, etc. & on-demand & Transient & Network, Pod, Stress, HTTP & \ding{51} & \ding{51} & \ding{51} \\
        VECROsim\cite{vecrosim} & Flexible & Flexible & Go, Python & on-demand & Transient & Network, Pod, Stress & \ding{51} & - & - \\
        TrainTicket\cite{trainticket} & M(41) & Train ticket booking & Java, JavaScript & Hard-coded & Permanent & - & \ding{51} & \ding{51} & \ding{51} \\
        DeathStarBench\cite{deathstar} & M(21-41) & Social network, banking, etc. & C, C++, etc. & - & - & - & \ding{51} & \ding{51} & \ding{51} \\
        Theodolite\cite{theodolite} & M($\sim$10) & Streaming & Java, Kotlin & - & - & - & \ding{51} & \ding{51} & \ding{51} \\
        $\mu$Bench\cite{mubench} & Flexible & Flexible & Python & on-demand & Transient & Network, Disk, Stress & \ding{51} & \ding{51} & \ding{51} \\
        \bottomrule
        \end{tabular} 
        \begin{tablenotes}[para]
            \item[1] `-' means this microservice benchmark does not support this feature
            \item[2] Medium (M)
            \item[3] `-' means this microservice benchmark does not collect this type of data
        \end{tablenotes}
        \end{threeparttable}
    }
    \label{table:benchmark_system}
\end{table*}

==> tables/container_level_metric.tex <==
\begin{table}
    \caption{Container-level Metrics}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{lll}
        \toprule
        \textbf{Name} & \textbf{Unit} & \textbf{Description} \\
        \midrule
         cpu\_usage\_seconds\_total  & Seconds & Total cumulative CPU time used. \\
         cpu\_user\_seconds\_total  & Seconds & Total time CPU spent in user mode. \\
         cpu\_system\_seconds\_total  & Seconds & Total time CPU spent in system mode. \\
         cpu\_cfs\_throttled\_seconds\_total  & Seconds & Total time processes were throttled by CFS. \\
         cpu\_cfs\_throttled\_periods\_total  & Periods & Number of periods processes were throttled. \\
         cpu\_cfs\_periods\_total  & Periods & Total number of observed CFS periods. \\
         memory\_cache  & Bytes & Memory used by the cache. \\
         memory\_usage\_bytes  & Bytes & Total memory usage. \\
         memory\_working\_set\_bytes  & Bytes & Memory being used and not easily available. \\
         spec\_cpu\_period  & Microseconds & The CPU period for the CFS scheduler. \\
         spec\_cpu\_quota  & Microseconds & The CPU quota for the CFS scheduler. \\
         spec\_memory\_limit\_bytes  & Bytes & Maximum configurable memory for a container. \\
         spec\_cpu\_shares  & Relative Units & CPU shares relative to other containers. \\
         threads  & Count & Current number of threads in use. \\
         threads\_max  & Count & Maximum number of threads used. \\
         network\_receive\_bytes\_total & Bytes & Total number of bytes received by network interfaces. \\
         network\_transmit\_bytes\_total & Bytes &  Total number of bytes transmitted by network interfaces. \\
        \bottomrule
        \end{tabular}
    }
    \label{table:container_metrics}
\end{table}

==> tables/dataset_scenario.tex <==
\begin{table*}[htb]
    \centering
    \caption{Generated Fault Cases}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{llllll}
        \toprule
        \textbf{Case} & \textbf{Fault Type} & \textbf{Start Time} & \textbf{Duration} & \textbf{Description} & \textbf{Fault Root Cause} \\
        \midrule
        \multirow{3}{*}{1} & Network Loss & 02:00 & 15 min & 50\% chance of packet loss from recommendationservice-1 to productcatalogservice-1 & recommendationservice-1 \\
                           & Network Delay & 06:35 & 13 min & 2000 ms delay in the network from cartservice-2 to redis-cart-0 & cartservice-2 \\
                           & HTTP Request Delay & 09:23 & 12 min & All requests on port 5050 of checkoutservice-1 experience a 3000 ms delay & checkoutservice-1 \\
        \multirow{2}{*}{2} & CPU Stress & 03:20 & 9 min & CPU load reaches 100\% & paymentservice-1 \\
                           & Memory Stress & 10:50 & 11 min & Memory usage of emailservice-2 reaches 100\% & emailservice-2 \\
        \multirow{2}{*}{3} & Pod Failure & 16:07 & 10 min & frontend-0 stops running & frontend-0 \\
                           & Pod Failure & 20:49 & 14 min & currencyservice-0 stops running & currencyservice-0 \\
        \bottomrule
        \end{tabular}
    }
    \label{table:dataset_scenario}
\end{table*}


==> tables/evaluation_metric.tex <==
\begin{table*}
    \centering
    \caption{Format of Evaluation Metrics}
    \resizebox{\linewidth}{!}{
        \begin{threeparttable}
        \begin{tabular}{ll}
        \toprule
        \textbf{Evaluation Metric} & \textbf{Format} \\
        \midrule
        Precision, Recall, F1-score & \{prf: \{i\tnote{1}: \{precision: xx, recall: xx, f1-score: xx\}\}, epoch\tnote{2}: xx\} \\
        Accuracy@k & \{accuracy@k:\{i:\{top1: xx, top2: xx, top3: xx, top4: xx, top5: xx\}\}, epoch: xx\} \\
        Top@k & \{top@k: \{i: \{top1: xx, top2: xx, top3: xx, top4: xx, top5: xx\}\}, epoch: xx\} \\
        \bottomrule
        \end{tabular}
        \begin{tablenotes}[para]
            \item[1] `i' means the result of the i-th epoch
            \item[2] `epoch' is the parameter that user sets before running
        \end{tablenotes}
        \end{threeparttable}
    }
    \label{tab:evaluation_metrics}
\end{table*}

==> tables/service_level_metric.tex <==
\begin{table}
    \centering
    \caption{Service-level Metrics}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{llllll|l|llllll}
        \toprule
        \textbf{Name} & \textbf{Unit} & \textbf{Description} \\
        \midrule
        istio\_requests\_total & Count & Total number of Istio requests. \\
        istio\_request\_duration\_milliseconds\_sum & Milliseconds & Sum of request durations in milliseconds. \\
        istio\_request\_bytes\_sum & Bytes & Total sum of request bytes. \\
        istio\_response\_bytes\_sum & Bytes & Total sum of response bytes. \\
        istio\_request\_messages\_total & Count & Total number of request messages. \\
        istio\_response\_messages\_total & Count & Total number of response messages. \\
        istio\_tcp\_sent\_bytes\_total & Bytes & Total number of TCP bytes sent. \\
        istio\_tcp\_received\_bytes\_total & Bytes & Total number of TCP bytes received. \\
        istio\_tcp\_connections\_opened\_total & Count & Total number of opened TCP connections. \\
        istio\_tcp\_connections\_closed\_total & Count & Total number of closed TCP connections. \\
        \bottomrule
        \end{tabular}
    }
    \label{table:service_metrics}
\end{table}
